Approximative lookup-tables and arbitrary function rotations for facilitating NISQ-implementations of the HHL and beyond

Many promising applications of quantum computing with a provable speedup center around the HHL algorithm. Due to restrictions on the hardware and its significant demand on qubits and gates in known implementations, its execution is prohibitive on near-term quantum computers. Aiming to facilitate such NISQ-implementations, we propose a novel circuit approximation technique that enhances the arithmetic subroutines in the HHL, which resemble a particularly resource-demanding component in small-scale settings. For this, we provide a description of the algorithmic implementation of space-efficient rotations of polynomial functions that do not demand explicit arithmetic calculations inside the quantum circuit. We show how these types of circuits can be reduced in depth by providing a simple and powerful approximation technique. Moreover, we provide an algorithm that converts lookup-tables for arbitrary function rotations into a structure that allows an application of the approximation technique. This allows implementing approximate rotation circuits for many polynomial and non-polynomial functions. Experimental results obtained for realistic early-application dimensions show significant improvements compared to the state-of-the-art, yielding small circuits while achieving good approximations.

==> txt/tables/haener.tex <==
\begin{table}
\centering
\caption{Häner.}

\begin{tabular}{l|c|c}
$d = 1$ & Toffoli & Ancilla  \\
\hline
$n=8$ & 64 & 9  \\ 

\hline
$n=10$ & 80 & 11  \\ 

\hline
$n=12$ & 96 & 13  \\ \\

$d = 3$ & Toffoli & Ancilla  \\
\hline
$n=8$ & 2*353 & 33  \\ 

\hline
$n=10$ & 2*544 & 41  \\ 

\hline
$n=12$ & 2*771 & 49  \\ 
\end{tabular}
\end{table}

==> txt/tables/near_optimal_accuracy_circuit_depths.tex <==
\begin{table}
    \centering
    \caption{The lookup-table Toffoli counts required for reaching near-machine precision for different polynomial and non-polynomial functions.}
    \label{tab:near_optimal_accuracy_circuit_depth}
    \begin{tabular}{c|c|c|c|c}
        $n$ & $x^3$ & $x^5$ & $\arcsin(x)$ & Worst-case for any function\\ \hline
        6 & 110 & 248 & 258 & 258 \\
        7 & 182 & 560 & 642 & 642 \\
        8 & 280 & 1148 & 1538 & 1538 \\
        9 & 408 & 2172 & 3586 & 3586  \\
        10 & 570 & 3846 & 8194 & 8194\\
        11 & 770 & 6446 & 18434 & 18434 \\
        12 & 1012 & 10318 & 40962 & 40962
    \end{tabular}
\end{table}
